XALP-completeness of Parameterized Problems on Planar Graphs

The class XNLP consists of (parameterized) problems that can be solved nondeterministically in $f(k)n^{O(1)}$ time and $f(k)\log n$ space, where $n$ is the size of the input instance and $k$ the parameter. The class XALP consists of problems that can be solved in the above time and space with access to an additional stack. These two classes are a "natural home" for many standard graph problems and their generalizations. In this paper, we show the hardness of several problems on planar graphs, parameterized by outerplanarity, treewidth and pathwidth, thus strengthening several existing results. In particular, we show the XALP-completeness of the following problems parameterized by outerplanarity: All-or-Nothing Flow, Target Outdegree Orientation, Capacitated (Red-Blue) Dominating Set, Target Set Selections etc. We also show the XNLP-completeness of Scattered Set parameterized by pathwidth and XALP-completeness parameterized by treewidth and outerplanarity.

==> figures/circulatingorientation.tex <==
\subsection{Circulating Orientation}
A special case of the \textsc{Target Outdegree Orientation} problem
is \textsc{Circulating Orientation}. The problem is XNLP-complete
with pathwidth as parameter~\cite{BodlaenderCW22a} and XALP-complete
with treewidth as parameter~\cite{BodlaenderGJPP22a}. Jansen et al.~\cite{JansenKKLMS23} showed that the problem is W[1]-hard for
planar graphs with treewidth as parameter. Here, we give a stronger result, and show that the problem is XNLP-hard for planar graphs
with outerplanarity and pathwidth as parameter, by observing a
property of the graphs constructed in the XNLP-hardness proof for
\textsc{All-or-Nothing Flow}.

Given an undirected graph $G=(V,E)$ with each edge a capacity
$c(e)\in \mathbb{N}$, an orientation of $G$ is said to be
\emph{circulating} if for each $v\in V$, the total weight of
all edges that have $v$ as head in the orientation equals the
total weight of all edges that have $v$ as tail in the orientation.
(The name is inspired from circulations from flow theory: a circulation is a flow with all vertices having equal inflow and outflow.)

\defproblem{\textsc{Circulating Orientation}}{$G = (V,E)$, with each edge a capacity $c(e)\in \mathbb{N}$}{Does $G$ have a circulating orientation?}

Note that the \textsc{Circulating Orientation} problem is
the special case of \textsc{Target Outdegree Orientation}
where all vertices $v\in V$ have $t(v)$ equal to the sum of all
weights of edges incident to $v$ divided by $2$.

\begin{observation}
    A graph $G$ constructed by the XNLP-hardness proof for 
    \textsc{All-or-Nothing Flow} from Section TODO has the following 
    property: we can add a simple cycle $C$ to $G$ that contains all vertices
    in $G$ with degree more than 2, such that $G+C$ is planar and
    has outerplanarity at most 1 larger than the outerplanarity of
    $G$.
\end{observation}
